A Multi-Scale A Contrario method for Unsupervised Image Anomaly Detection

Anomalies can be defined as any non-random structure which deviates from normality. Anomaly detection methods reported in the literature are numerous and diverse, as what is considered anomalous usually varies depending on particular scenarios and applications. In this work we propose an a contrario framework to detect anomalies in images applying statistical analysis to feature maps obtained via convolutions. We evaluate filters learned from the image under analysis via patch PCA, Gabor filters and the feature maps obtained from a pre-trained deep neural network (Resnet). The proposed method is multi-scale and fully unsupervised and is able to detect anomalies in a wide variety of scenarios. While the end goal of this work is the detection of subtle defects in leather samples for the automotive industry, we show that the same algorithm achieves state of the art results in public anomalies datasets.

==> NFA _ ICMLA/plot_cracks.tex <==
% \vspace{-10pt}
\captionsetup{position=top}
\begin{figure}[tb]

\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0000.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0003.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0007.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/024_0008.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/030_0002.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/054_0003.jpg}} \hfill \\[-20px]

    \caption{Comparison of different method over the Cracks Dataset. (a) image, (b) label, (c) ours, (d) DRFI, (e) GBVS, (f) SALICON, (g) All Terrain}
    \vspace{-10pt}
    \label{fig:results-cracks}
\end{figure}
\captionsetup{position=bottom}

==> NFA _ ICMLA/plot_example_images.tex <==
\captionsetup{position=top}
\begin{figure}[tb]

\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/01.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/02.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/03.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/04.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/05.jpeg}} \hfill \\[-17px]

\captionsetup{position=bottom}
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/06.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/07.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/08.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/09.jpeg}} \hfill
\subfloat[]{\includegraphics[width=0.192\linewidth]{pics/example_images/10.jpeg}} \hfill \\[-10px]
    \caption{[Best viewed in color] Motivating application: defect detection in leather samples. Example images showing the diversity of samples. Image (a) and (b) correspond to the same texture, with different engraving strength. The defect present in (b) may not be considered an anomaly if it was in (a). Images (c), (d) and (e) are examples of different textures. (f) and (g) show different color possibilities, and (h), (i) and (j) correspond to the down side of leather samples.}
    \vspace{-18pt}
    \label{fig:example-images}
\end{figure}

==> NFA _ ICMLA/plot_ipol.tex <==
\vspace{-10pt}
\captionsetup{position=top}
\begin{figure}[tb]

\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/images/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/bird.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/field3_bw.jpg}} \hfill \\[-20px]
    
    \caption{Comparison of the same methods mentioned over sample interesting images (excluding All Terrain algorithm, which was specific for cracks). (a) image, (b) Our NFA map, (c) Our segmentation using NFA=0 as threshold, (d) DRFI, (e) GBVS, (f) SALICON}
    \vspace{-10pt}
    \label{fig:results-ipol}
\end{figure}
\captionsetup{position=bottom}

==> NFA _ ICMLA/table_related_work.tex <==

% {\setlength{\tabcolsep}{1em} {\renewcommand{\arraystretch}{1.}%
% \begin{table}[b]
% \vspace{-15pt}
% \caption{}\label{}
% \vspace{-5pt}
% \centering
\begin{table*}[t]
\caption{Related work comparison showing some of the key elements of each method: how they generate the final anomaly map, whether if they use some pre-trained network or not, how is the usage of normal and abnormal images, the kind of supervision, if they solve a proxy task and the way to achieve the multi-scale analysis.}
\label{tab:related-work}
\vspace{-10pt}
\scriptsize
\begin{center}
    \begin{tabular}{m{7em}|m{17em}|m{3em}|m{5em}|m{3.3em}|m{2em}|m{4.5em}|m{5.5em}|m{9.4em}}
        
        {\bfseries Method} & {\bfseries Anomaly map} & {\bfseries Pre-trained} & {\bfseries Normal images usage} & {\bfseries Anomaly img use}  & {\bfseries Thr} & {\bfseries Supervision} & {\bfseries Proxy task} & {\bfseries Multi-Scale}\\
        \hline  
        
\textbf{TextureInsp}~\cite{text} & Negative log-likelihood for trained GMM & No & Fit GMM & No & No & Sup. & No & 4-layer pyramid \\ 
\textbf{SPADE}~\cite{spade} & Euclidean distance to normal samples & Resnet & kNN & No & No & Sup. & No & DNN scales \\
\textbf{DictSimilarity}~\cite{dict} & Distance to normality & Yes & Build dict. & No & No & Sup. & No & Different patch sizes \\ 
\textbf{FCDD}~\cite{fcdd} & Activation layer from network & No & FCN & Yes & No & Sup. & No & DNN scales \\ 
\textbf{PaDiM}~\cite{padim} & Mahalanobis distance by patch & Resnet & Mah. dist. & No & No & Self-Sup. & No & DNN scales \\
\textbf{PatchSVDD}~\cite{patch-svdd} & Distance to normal samples & No & Encoder & No & No & Self-Sup. & Patch-gather & Arch design \\ 
\textbf{RotDet}~\cite{rotnet} & KDE at each patch location & No & DNN & No & No & Self-Sup. & Rotation & DNN scales \\ 
\textbf{STPM}~\cite{student-teacher} & Student-teacher L2 distance & Resnet & Student net & No & No & Self-Sup. & No & DNN scales \\ 
\textbf{DetInNoise}~\cite{ehret2019reduce} & Log-NFA map & Optional & No & No & Yes & UnSup. & No & Downsampled images \\ 
\hline
\textbf{SSIM-AE}~\cite{bergmann-ssim} & Reconstruction error & No & AE & No & No & Self-Sup. & No & AE architecture \\ 
\textbf{AnoGan}~\cite{anogan} & Reconstruction error & No & GAN & No & No & Self-Sup. & No & GAN architecture \\ 
\textbf{InTra}~\cite{intra} & Reconstruction error & No & Transformer & No & No & Self-Sup. & Inpainting & Downsampled images \\ 
\textbf{CutPaste}~\cite{cutpaste} & One class over representation & No & DNN & No & No & Self-Sup. & Cut-Paste & Replicating \\ 
\textbf{DFR}~\cite{dfr} & Reconstruction error & VGG19 & VAE & No & No & Self-Sup. & No & DNN scales \\ 
%\textbf{IGD}~\cite{igd} & Local and global reconstruction error & Optional & AE & No & No & Self-Sup. & No & Whole image + patches \\ 
% @article{igd,
%   title={Unsupervised Anomaly Detection with Multi-scale Interpolated Gaussian Descriptors},
%   author={Chen, Yuanhong and Tian, Yu and Pang, Guansong and Carneiro, Gustavo},
%   journal={arXiv preprint arXiv:2101.10043},
%   year={2021}
% }
\hline 
\textbf{GBVS}~\cite{gbvs-harel2007graph} & Equilibrium distribution of markov chain & No & No & No & No & UnSup. & No & Downsampled images \\ 
\textbf{SALICON}~\cite{salicon-huang2015salicon} & Activation layer from network & No & No & Yes & No & Sup. & No & Arch design \\ 
\textbf{DRFI}~\cite{drfi-jiang2013salient} & RF Regression & No & No & Yes & No & Sup. & No & Multi-Level segmentat. \\ 
\hline 
\textbf{Ours} & Log-NFA map & Optional & No & No & Yes & UnSup. & No & Downsampled images \\ 

    \end{tabular}
\end{center}
\normalsize
\vspace{-15pt}
\end{table*}
% \end{table}
% }}

==> NFA _ ICMLA/table_results.tex <==
% {\setlength{\tabcolsep}{0.5em} {\renewcommand{\arraystretch}{1.3}%
% \begin{table}[t]
% \vspace{-15pt}
% \caption{Area under the receiver operating characteristic curve (ROC AUC). Best two cores in boldface}\label{tabresultsmvtec}
% \vspace{-5pt}
% \centering
%     \begin{tabular}{l|l|l|l|l|l|l}
%         % \hline
%         {\bfseries Method} & {\bfseries Carpet} & {\bfseries Grid} & {\bfseries Leather} & {\bfseries Tile} & {\bfseries Wood} & {\bfseries Mean} \\ 
%         \hline
% AE-SSIM~\cite{bergmann-ssim} & 0.87 & \textbf{0.94} & 0.78 & 0.59 & 0.73 & 0.78 \\ 
% AE-L2~\cite{bergmann-ssim} & 0.59 & 0.90 & 0.75 & 0.51 & 0.73 & 0.70 \\ 
% AnoGan~\cite{anogan} & 0.54 & 0.58 & 0.64 & 0.50 & 0.62 & 0.58 \\ 
% CNN Dict~\cite{dict} & 0.72 & 0.59 & 0.87 & \textbf{0.93} & \textbf{0.91} & 0.80 \\ 
% Text insp.~\cite{text} & \textbf{0.88} & 0.72 & 0.97 & 0.41 & 0.78 & 0.75 \\ \hline
% DRFI~\cite{drfi-jiang2013salient} & 0.72 & 0.58 & 0.68 & 0.72 & 0.67 & 0.67 \\ 
% GBVS~\cite{gbvs-harel2007graph} & 0.45 & 0.73 & 0.86 & 0.49 & 0.79 & 0.66 \\ 
% Salicon~\cite{salicon-huang2015salicon} & 0.53 & 0.79 & 0.76 & 0.40 & 0.72 & 0.64 \\ 
% Det in noise~\cite{ehret2019reduce} & 0.57 & 0.68 & 0.81 & 0.53 & 0.57 & 0.63 \\ \hline
% Ours-PCA & 0.76 & 0.88 & \textbf{0.98} & 0.69 & 0.86 & 0.83 \\ 
% Ours-PCA~\textsuperscript{\Cross} & 0.65 & 0.91 & 0.87 & \textbf{0.84} & \textbf{0.87} & 0.83 \\ 
% Ours-Gabor & 0.77 & 0.90 & 0.95 & 0.79 & \textbf{0.87} & \textbf{0.86} \\ 
% Ours-Gabor~\textsuperscript{\Cross} & 0.69 & 0.83 & 0.92 & 0.80 & 0.84 & 0.82 \\ 
% Ours-ResNet & \textbf{0.94} & \textbf{0.92} & \textbf{0.99} & 0.77 & 0.86 & \textbf{0.90} \\
%         % \hline
%         \end{tabular}
% \vspace{-10pt}
% \end{table}
% }}

{\setlength{\tabcolsep}{0.35em} {\renewcommand{\arraystretch}{1.2}%
\begin{table}[t]
% \vspace{-15pt}
\caption{Area under the receiver operating characteristic curve (ROC AUC). In red the best score, blue the second best and green the third. The ranking of the algorithms is done by sorting the performance and summing the positions for each algorithm. The one with lowest value is the best.}\label{tabresultsmvtec}
\vspace{-5pt}
\centering
    \begin{tabular}{l|c|c|c|c|c|c|c}
        % \hline
        {\bfseries Method} & {\bfseries Carpet} & {\bfseries Grid} & {\bfseries Leather} & {\bfseries Tile} & {\bfseries Wood} & {\bfseries Mean} & {\bfseries Rank} \\ 
        \hline
AE-SSIM~\cite{bergmann-ssim} & \textcolor{green}{\textbf{0.87}} & \textcolor{red}{\textbf{0.94}} & 0.78 & 0.59 & 0.73 & 0.78 & 7\\ 
AE-L2~\cite{bergmann-ssim} & 0.59 & 0.90 & 0.75 & 0.51 & 0.73 & 0.70 & 9\\ 
AnoGan~\cite{anogan} & 0.54 & 0.58 & 0.64 & 0.50 & 0.62 & 0.58 & 14\\ 
CNN Dict~\cite{dict} & 0.72 & 0.59 & 0.87 & \textcolor{red}{\textbf{0.93}} & \textcolor{red}{\textbf{0.91}} & 0.80 & 5\\ 
Text insp.~\cite{text} & \textcolor{blue}{\textbf{0.88}} & 0.72 & \textcolor{green}{\textbf{0.97}} & 0.41 & 0.78 & 0.75 & 8\\ \hline
DRFI~\cite{drfi-jiang2013salient} & 0.72 & 0.58 & 0.68 & 0.72 & 0.67 & 0.67 & 10\\ 
GBVS~\cite{gbvs-harel2007graph} & 0.45 & 0.73 & 0.86 & 0.49 & 0.79 & 0.66 & 11\\ 
Salicon~\cite{salicon-huang2015salicon} & 0.53 & 0.79 & 0.76 & 0.40 & 0.72 & 0.64 & 13\\ 
DetNoise~\cite{ehret2019reduce} & 0.57 & 0.68 & 0.81 & 0.53 & 0.57 & 0.63 & 12 \\ \hline
Ours-PCA & 0.76 & 0.88 & \textcolor{blue}{\textbf{0.98}} & 0.69 & \textcolor{green}{\textbf{0.86}} & \textcolor{green}{\textbf{0.83}} & 4\\ 
Ours-PCA~\textsuperscript{\Cross} & 0.65 & \textcolor{green}{\textbf{0.91}} & 0.87 & \textcolor{blue}{\textbf{0.84}} & \textcolor{blue}{\textbf{0.87}} & \textcolor{green}{\textbf{0.83}} & \textcolor{green}{\textbf{3}}\\ 
Ours-Gabor & 0.77 & 0.90 & 0.95 & 0.79 & \textcolor{blue}{\textbf{0.87}} & \textcolor{blue}{\textbf{0.86}} & \textcolor{blue}{\textbf{2}}\\ 
Ours-Gabor~\textsuperscript{\Cross} & 0.69 & 0.83 & 0.92 & \textcolor{green}{\textbf{0.80}} & 0.84 & 0.82 & 6\\ 
Ours-ResNet & \textcolor{red}{\textbf{0.94}} & \textcolor{blue}{\textbf{0.92}} & \textcolor{red}{\textbf{0.99}} & 0.77 & 0.86 & \textcolor{red}{\textbf{0.90}} & \textcolor{red}{\textbf{1}}\\
        % \hline
        \end{tabular}
\vspace{-10pt}
\end{table}
}}

% \begin{table*}[t]
% % \vspace{-15pt}
% \caption{Area under the receiver operating characteristic curve (ROC AUC). Best two cores in boldface.}\label{tabresultsmvtec}
% \vspace{-5pt}
% \centering
%     \begin{tabularx}{\linewidth}{X X X X X X X X X X X X X X X}
% \toprule
% \textbf{Method} & AE$_{ssim}$ \cite{bergmann-ssim} & AE$_{L2}$ \cite{bergmann-ssim} & AnoGan \cite{anogan} & CnnDict \cite{dict} & TexInsp \cite{text} & DRFI \cite{drfi-jiang2013salient} & GBVS \cite{gbvs-harel2007graph} & Salicon \cite{salicon-huang2015salicon} & DetNoise \cite{ehret2019reduce} & Ours-PCA & Ours-PCA~	\textsuperscript{\Cross} & Ours-Gabor & Ours-Gabor\textsuperscript{\Cross} & Ours-ResNet\\ 
% \midrule
% \textbf{Carpet} & 0.87 & 0.59 & 0.54 & 0.72 & \textbf{0.88} & 0.72 & 0.45 & 0.53 & 0.57 & 0.76 & 0.65 & 0.77 & 0.69 & \textbf{0.94}\\
% \textbf{Grid} & \textbf{0.94} & 0.90 & 0.58 & 0.59 & 0.72 & 0.58 & 0.73 & 0.79 & 0.68 & 0.88 & 0.91 & 0.90 & 0.83 & \textbf{0.92}\\
% \textbf{Leather} & 0.78 & 0.75 & 0.64 & 0.87 & 0.97 & 0.68 & 0.86 & 0.76 & 0.81 & \textbf{0.98} & 0.87 & 0.95 & 0.92 & \textbf{0.99}\\
% \textbf{Tile} & 0.59 & 0.51 & 0.50 & \textbf{0.93} & 0.41 & 0.72 & 0.49 & 0.40 & 0.53 & 0.69 & \textbf{0.84} & 0.79 & 0.80 & 0.77\\
% \textbf{Wood} & 0.73 & 0.73 & 0.62 & \textbf{0.91} & 0.78 & 0.67 & 0.79 & 0.72 & 0.57 & 0.86 & \textbf{0.87} & \textbf{0.87} & 0.84 & 0.86\\
% \midrule
% \textbf{Mean} & 0.78  & 0.70  & 0.58  & 0.80  & 0.75  & 0.67  & 0.66  & 0.64  & 0.63  & 0.83  & 0.83  & \textbf{0.86}  & 0.82  & \textbf{0.90}\\ 
% \bottomrule
%         \end{tabularx}
% \vspace{-10pt}
% \end{table*}

% \begin{table*}[t]
% % \vspace{-15pt}
% \caption{Area under the receiver operating characteristic curve (ROC AUC). In red the best score, blue the second best and green the third. The ranking of the algorithms is done by sorting the performance and summing the positions for each algorithm. The one with lowest value is the best.}\label{tabresultsmvtec}
% \vspace{-5pt}
% \centering
%     \begin{tabularx}{\linewidth}{X X X X X X X X X X X X X X X}
% \toprule
% \textbf{Method} & AE$_{ssim}$ \cite{bergmann-ssim} & AE$_{L2}$ \cite{bergmann-ssim} & AnoGan \cite{anogan} & CnnDict \cite{dict} & TexInsp \cite{text} & DRFI \cite{drfi-jiang2013salient} & GBVS \cite{gbvs-harel2007graph} & Salicon \cite{salicon-huang2015salicon} & DetNoise \cite{ehret2019reduce} & Ours-PCA & Ours-PCA~	\textsuperscript{\Cross} & Ours-Gabor & Ours-Gabor\textsuperscript{\Cross} & Ours-ResNet\\ 
% \midrule
% \textbf{Carpet} &  \textcolor{green}{\textbf{0.87}} &  0.59 &  0.54 &  0.72 &  \textcolor{blue}{\textbf{0.88}} &  0.72 &  0.45 &  0.53 &  0.57 &  0.76 &  0.65 &  0.77 &  0.69 &  \textcolor{red}{\textbf{0.94}}\\
% \textbf{Grid} &  \textcolor{red}{\textbf{0.94}} &  0.90 &  0.58 &  0.59 &  0.72 &  0.58 &  0.73 &  0.79 &  0.68 &  0.88 &  \textcolor{green}{\textbf{0.91}} &  0.90 &  0.83 &  \textcolor{blue}{\textbf{0.92}}\\
% \textbf{Leather} &  0.78 &  0.75 &  0.64 &  0.87 &  \textcolor{green}{\textbf{0.97}} &  0.68 &  0.86 &  0.76 &  0.81 &  \textcolor{blue}{\textbf{0.98}} &  0.87 &  0.95 &  0.92 &  \textcolor{red}{\textbf{0.99}}\\
% \textbf{Tile} &  0.59 &  0.51 &  0.50 &  \textcolor{red}{\textbf{0.93}} &  0.41 &  0.72 &  0.49 &  0.40 &  0.53 &  0.69 &  \textcolor{blue}{\textbf{0.84}} &  0.79 &  \textcolor{green}{\textbf{0.80}} &  0.77\\
% \textbf{Wood} &  0.73 &  0.73 &  0.62 &  \textcolor{red}{\textbf{0.91}} &  0.78 &  0.67 &  0.79 &  0.72 &  0.57 &  \textcolor{green}{\textbf{0.86}} &  \textcolor{blue}{\textbf{0.87}} &  \textcolor{blue}{\textbf{0.87}} &  0.84 &  0.86\\
% \midrule
% \textbf{Mean} &  0.78 &  0.70 &  0.58 &  0.80 &  0.75 \  &  0.67 &  0.66 &  0.64 &  0.63 \  &  \textcolor{green}{\textbf{0.83}} &  \textcolor{green}{\textbf{0.83}} &  \textcolor{blue}{\textbf{0.86}} &  0.82 &  \textcolor{red}{\textbf{0.90}}\\
% \midrule
% \textbf{Ranking} & 7 & 9 & 14 & 5 & 8 & 10 & 11 & 13 & 12 & 4 & \textcolor{green}{\textbf{3}} & \textcolor{blue}{\textbf{2}} & 6 & \textcolor{red}{\textbf{1}}\\
% \bottomrule
%         \end{tabularx}
% % \vspace{-10pt}
% \end{table*}

==> plot_cracks.tex <==
% \vspace{-10pt}
\captionsetup{position=top}
\begin{figure}[tb]

\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0000.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0000.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0003.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/001_0007.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/001_0007.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/024_0008.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/024_0008.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/030_0002.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/030_0002.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/images/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/labels/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/ours_blob_gabor/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/drfi/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/gbvs/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/salicon/054_0003.jpg}} \hfill
\subfloat{\includegraphics[width=0.138\linewidth]{pics/cracks/allterrain_augmented/054_0003.jpg}} \hfill \\[-20px]

    \caption{Comparison of different method over the Cracks Dataset. (a) image, (b) label, (c) ours, (d) DRFI, (e) GBVS, (f) SALICON, (g) All Terrain}
    \vspace{-10pt}
    \label{fig:results-cracks}
\end{figure}
\captionsetup{position=bottom}

==> plot_ipol.tex <==
\vspace{-10pt}
\captionsetup{position=top}
\begin{figure}[tb]

\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/images/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill
\subfloat[]{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/55fff9bfc4007c65aaff1b2cad9237a411e703bd.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/693ca1ea0ca72e9d2c81e3ae5909314ca00cb0b7.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/785e7cf1731258e05e4cf843bea1ffcd3ddc52a7.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/9c577c528e24499626b18e60584bdb00a776827e.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/bird.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/bird.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/d779a25c72c3f3318d1402af822068ceb7a5c5ae.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/e634e2f23efae2af8447a5a29ef1a979f8a317fe.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/f4252df6758563293bdbc6a7db346bbb922778cf.jpg}} \hfill \\[-20px]

\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/images/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_nfa/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/ours_det/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/drfi/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/gbvs/field3_bw.jpg}} \hfill
\subfloat{\includegraphics[width=0.162\linewidth]{pics/ipol/salicon/field3_bw.jpg}} \hfill \\[-20px]
    
    \caption{Comparison of the same methods mentioned over sample interesting images (excluding All Terrain algorithm, which was specific for cracks). (a) image, (b) Our NFA map, (c) Our segmentation using NFA=0 as threshold, (d) DRFI, (e) GBVS, (f) SALICON}
    \vspace{-10pt}
    \label{fig:results-ipol}
\end{figure}
\captionsetup{position=bottom}
